A Minimax Approach to Ad Hoc Teamwork

We propose a minimax-Bayes approach to Ad Hoc Teamwork (AHT) that optimizes policies against an adversarial prior over partners, explicitly accounting for uncertainty about partners at time of deployment. Unlike existing methods that assume a specific distribution over partners, our approach improves worst-case performance guarantees. Extensive experiments, including evaluations on coordinated cooking tasks from the Melting Pot suite, show our method's superior robustness compared to self-play, fictitious play, and best response learning. Our work highlights the importance of selecting an appropriate training distribution over teammates to achieve robustness in AHT.

==> data/cooking/table_old.tex <==
\begin{table*}[t]
    %\small
    \setlength{\tabcolsep}{3pt}
    \centering
    \caption{Scores on the Collaborative Cooking environment training and test sets. The standard error is taken over three random seeds. The scores are aggregated over the two kitchen layouts.}
    \label{tab:cooking.train}
    \begin{tabular}{lccccc}\toprule
    & \multicolumn{5}{c}{$\scenarioset(\poptrain)$}\\
    \cmidrule(lr){2-6}
               & $\perf$ & p(wcu) & p(wcr) & $\wcu$ & $\wcr$ \\ \midrule
        MU & $\mathbf{266.9 {\scriptscriptstyle\pm 4.3}}$ & $\mathbf{23.1 {\scriptscriptstyle\pm 0.7}}$ & $\mathbf{24.5 {\scriptscriptstyle\pm 0.8}}$ & $\mathbf{225.3 {\scriptscriptstyle\pm 11.5}}$ & $266.0 {\scriptscriptstyle\pm 7.9}$ \\
        MR & $232.0 {\scriptscriptstyle\pm 18.6}$ & $19.9 {\scriptscriptstyle\pm 1.6}$ & $20.2 {\scriptscriptstyle\pm 1.4}$ & $144.3 {\scriptscriptstyle\pm 14.4}$ & $\mathbf{230.7 {\scriptscriptstyle\pm 28.2}}$ \\ \hdashline
        PBR & $209.7 {\scriptscriptstyle\pm 23.9}$ & $20.0 {\scriptscriptstyle\pm 1.7}$ & $18.4 {\scriptscriptstyle\pm 3.1}$ & $96.8 {\scriptscriptstyle\pm 13.4}$ & $357.6 {\scriptscriptstyle\pm 16.1}$ \\
        FP & $129.9 {\scriptscriptstyle\pm 13.9}$ & $7.9 {\scriptscriptstyle\pm 0.7}$ & $12.0 {\scriptscriptstyle\pm 1.1}$ & $0.2 {\scriptscriptstyle\pm 0.1}$ & $483.5 {\scriptscriptstyle\pm 16.1}$ \\
        SP & $124.8 {\scriptscriptstyle\pm 26.4}$ & $9.4 {\scriptscriptstyle\pm 2.8}$ & $11.8 {\scriptscriptstyle\pm 3.2}$ & $15.7 {\scriptscriptstyle\pm 10.5}$ & $460.8 {\scriptscriptstyle\pm 21.7}$ \\
        Random & $42.8 {\scriptscriptstyle\pm 0.0}$ & $6.7 {\scriptscriptstyle\pm 0.0}$ & $4.2 {\scriptscriptstyle\pm 0.0}$ & $0.0 {\scriptscriptstyle\pm 0.0}$ & $505.4 {\scriptscriptstyle\pm 0.0}$ \\
    \bottomrule
    \end{tabular}
\end{table*}

\begin{table}[t]
    %\small
    \setlength{\tabcolsep}{2.6pt}
    \centering
    \caption{Scores on the Collaborative Cooking environment test sets.}
    \label{tab:cooking.test}
    \begin{adjustbox}{center}

    \begin{tabular}{lcccccc}\toprule
    & \multicolumn{3}{c}{$\scenarioset(\poptest)$} & \multicolumn{3}{c}{$\setmeltingpot$}
    \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
               & $\perf$ & $U^-$ & $R^+$ & $\perf$ & $U^-$ & $R^+$ \\ \midrule
            MU & $\mathbf{195.7 {\scriptscriptstyle\pm 6.2}}$ & $\mathbf{66.0 {\scriptscriptstyle\pm 6.8}}$ & $266.4 {\scriptscriptstyle\pm 10.1}$ & $\mathbf{273.8 {\scriptscriptstyle\pm 4.9}}$ & $\mathbf{224.9 {\scriptscriptstyle\pm 7.1}}$ & $\mathbf{118.0 {\scriptscriptstyle\pm 7.1}}$ \\
            MR & $172.2 {\scriptscriptstyle\pm 15.4}$ & $65.1 {\scriptscriptstyle\pm 16.0}$ & $\mathbf{248.2 {\scriptscriptstyle\pm 28.4}}$ & $206.8 {\scriptscriptstyle\pm 12.6}$ & $148.7 {\scriptscriptstyle\pm 9.1}$ & $187.1 {\scriptscriptstyle\pm 13.0}$ \\ \hdashline
            PBR & $151.4 {\scriptscriptstyle\pm 19.5}$ & $33.6 {\scriptscriptstyle\pm 5.9}$ & $327.1 {\scriptscriptstyle\pm 14.0}$ & $171.8{\scriptscriptstyle \pm 21.1}$ & $106.3 {\scriptscriptstyle\pm 9.3}$ & $228.1 {\scriptscriptstyle\pm 5.8}$ \\
            FP & $152.2 {\scriptscriptstyle\pm 16.8}$ & $16.7 {\scriptscriptstyle\pm 11.7}$ & $369.7 {\scriptscriptstyle\pm 19.7}$ & $121.5 {\scriptscriptstyle\pm 15.7}$ & $40.7 {\scriptscriptstyle\pm 16.3}$ & $294.8 {\scriptscriptstyle\pm 10.7}$ \\
            SP & $117.4 {\scriptscriptstyle\pm 12.5}$ & $6.7 {\scriptscriptstyle\pm 3.5}$ & $367.5 {\scriptscriptstyle\pm 11.6}$ & $101.2 {\scriptscriptstyle\pm 17.8}$ & $29.0 {\scriptscriptstyle\pm 17.4}$ & $293.4 {\scriptscriptstyle\pm 14.5}$ \\
            Random & $32.2 {\scriptscriptstyle\pm 0.0}$ & $0.0 {\scriptscriptstyle\pm 0.0}$ & $445.0 {\scriptscriptstyle\pm 0.0}$ & $60.6 {\scriptscriptstyle\pm 0.0}$ & $0.0 {\scriptscriptstyle\pm 0.0}$ & $307.3 {\scriptscriptstyle\pm 0.0}$ \\ 
            PP-ACB & n/a & n/a & n/a & $82.4 {\scriptscriptstyle\pm 0.0}$ & $0.0 {\scriptscriptstyle\pm 0.0}$ & $307.3 {\scriptscriptstyle\pm 0.0}$ \\
            PP-OPRE & n/a & n/a & n/a & $102.3 {\scriptscriptstyle\pm 0.0}$ & $14.6 {\scriptscriptstyle\pm 0.0}$ & $292.7 {\scriptscriptstyle\pm 0.0}$ \\
            PP-VMPO & n/a & n/a & n/a & $78.6 {\scriptscriptstyle\pm 0.0}$ & $36.1 {\scriptscriptstyle\pm 0.0}$ & $306.7 {\scriptscriptstyle\pm 0.0}$ \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}


==> data/prisoners/scores.tex <==
T = 3

minimax_regret \[\Sigma(\mathcal{B}^\text{train})\] p= 9.170586968728966 U-= 0.8797296479180718
minimax_regret \[ \beta^*_U \] p= 0.8807468015945257
minimax_regret \[ \beta^*_R \] p= 11.00507128109278
minimax_regret $\Sigma(\mathcal{B^\text{test}})$ p= 7.538010814840733 U-= 0.9541583249892742
maximin_utility \[\Sigma(\mathcal{B}^\text{train})\] p= 6.822802287937026 U-= 2.98455101695313
maximin_utility \[ \beta^*_U \] p= 2.984856342981323
maximin_utility \[ \beta^*_R \] p= 8.095033749074236
maximin_utility $\Sigma(\mathcal{B^\text{test}})$ p= 8.653625009221974 U-= 3.0759885640445592
uniform \[\Sigma(\mathcal{B}^\text{train})\] p= 9.978438019738757 U-= 1.9644099753612752
uniform \[ \beta^*_U \] p= 1.965508961488689
uniform \[ \beta^*_R \] p= 10.656742399029682
uniform $\Sigma(\mathcal{B^\text{test}})$ p= 7.738694184714384 U-= 1.9857941413252556
self_play \[\Sigma(\mathcal{B}^\text{train})\] p= 9.689410350929743 U-= 0.5041721100171552
self_play \[ \beta^*_U \] p= 0.5053193067285658
self_play \[ \beta^*_R \] p= 11.681529548171698
self_play $\Sigma(\mathcal{B^\text{test}})$ p= 7.241413764014564 U-= 0.5211276419769548
fictitious_play \[\Sigma(\mathcal{B}^\text{train})\] p= 9.579904890526972 U-= 0.2152772403380261
fictitious_play \[ \beta^*_U \] p= 0.21644298867873668
fictitious_play \[ \beta^*_R \] p= 11.62029835117331
fictitious_play $\Sigma(\mathcal{B^\text{test}})$ p= 7.117685050149671 U-= 0.24395835971042126
random \[\Sigma(\mathcal{B}^\text{train})\] p= 8.1 U-= 1.5
random \[ \beta^*_U \] p= 1.5007
random \[ \beta^*_R \] p= 10.0998
random $\Sigma(\mathcal{B^\text{test}})$ p= 7.993009784858331 U-= 2.5232200142461
tft \[\Sigma(\mathcal{B}^\text{train})\] p= 9.998122973576741 U-= 1.999664721879585
tft \[ \beta^*_U \] p= 2.0006644871843475
tft \[ \beta^*_R \] p= 11.730357384915038
tft $\Sigma(\mathcal{B^\text{test}})$ p= 7.597949561850084 U-= 2.0119899018028566
cud \[\Sigma(\mathcal{B}^\text{train})\] p= 9.997721092902987 U-= 1.999664721879585
cud \[ \beta^*_U \] p= 2.000664554198154
cud \[ \beta^*_R \] p= 11.72927249301088
cud $\Sigma(\mathcal{B^\text{test}})$ p= 7.8451333382462645 U-= 2.0119923375266424
minimax_regret \[\Sigma(\mathcal{B}^\text{train})\] R+= 2.160156602781898
minimax_regret $\Sigma(\mathcal{B^\text{test}})$ R+= 8.62997607661227
maximin_utility \[\Sigma(\mathcal{B}^\text{train})\] R+= 8.92401143595544
maximin_utility $\Sigma(\mathcal{B^\text{test}})$ R+= 8.92401143595544
uniform \[\Sigma(\mathcal{B}^\text{train})\] R+= 2.9856565434931106
uniform $\Sigma(\mathcal{B^\text{test}})$ R+= 10.456555269880116
self_play \[\Sigma(\mathcal{B}^\text{train})\] R+= 2.991593297624304
self_play $\Sigma(\mathcal{B^\text{test}})$ R+= 10.644373606023326
fictitious_play \[\Sigma(\mathcal{B}^\text{train})\] R+= 2.9426243109970045
fictitious_play $\Sigma(\mathcal{B^\text{test}})$ R+= 10.650542831190739
random \[\Sigma(\mathcal{B}^\text{train})\] R+= 4.5
random $\Sigma(\mathcal{B^\text{test}})$ R+= 4.5
tft \[\Sigma(\mathcal{B}^\text{train})\] R+= 2.99899360381829
tft $\Sigma(\mathcal{B^\text{test}})$ R+= 9.926894589184558
cud \[\Sigma(\mathcal{B}^\text{train})\] R+= 2.9979883405230137
cud $\Sigma(\mathcal{B^\text{test}})$ R+= 9.922819534408987


==> data/prisoners/table_t3_old.tex <==
\begin{table}[t]
    %\small
    \setlength{\tabcolsep}{6pt}
    \centering
    \caption{
    Scores on the repeated Prisoner's Dilemma. A higher value is desired for performance ($p$, set average utility) and worst-case utility ($U^-$), while a lower worst-case regret ($R^+$) is better. $\perf(\beta)$ corresponds to the utility w.r.t.\ a specific distribution $\beta$, rather than the average as in \eqref{eq:metrics.performance}.}
    \label{tab:prisoner.train}
    \begin{tabular}{lcccccccc}\toprule
    & \multicolumn{5}{c}{$\scenarioset(\poptrain)$} & \multicolumn{3}{c}{$\scenarioset(\poptest)$}\\
    \cmidrule(lr){2-6}\cmidrule(lr){7-9}
               & $\perf$  & $\perf(\maximinprior)$ & $\perf(\minimaxprior)$ & $U^-$ & $R^+$ & $\perf$ & $U^-$ & $R^+$ \\ \midrule
        MU  & $7.69$ & $\mathbf{3.00}$ & $5.77$ & $\mathbf{3.00}$ & $9.00$ & $\mathbf{8.34}$ & $\mathbf{3.00}$ & $9.00$\\
        MR  & $8.23$ & $2.26$ & $\mathbf{6.00}$ & $2.26$ & $\mathbf{3.79}$ & $7.96$ & $2.78$ & $\mathbf{4.35}$\\ \hdashline
        PBR  & $\mathbf{8.54}$ & $2.00$ & $\mathbf{6.00}$ & $2.00$ & $4.97$ & $8.07$ & $2.48$ & $5.63$\\
        FP & $7.06$ & $0.14$ & $5.11$ & $0.14$ & $10.56$ & $6.33$ & $0.56$ & $9.96$\\
        SP  & $7.25$ & $0.47$ & $5.29$ & $0.47$ & $10.19$ & $6.49$ & $0.86$ & $9.65$\\
        %TfT  & $\mathbf{10.0}$ & $2.00$ & $11.73$ & $2.00$ & $3.00$ & $7.60$ & $2.01$ & $?$\\
        %CuD  & $\mathbf{10.0}$ & $2.00$ & $11.73$ & $2.00$ & $3.00$ & $7.85$ & $2.01$ & $?$\\
        Random & $7.40$ & $1.50$ & $5.50$ & $1.50$ & $5.50$ & $7.47$ & $2.18$ & $5.20$\\
    \bottomrule
    \end{tabular}
\end{table}

==> sections/bf_sgda.tex <==
% talk about the clipping idea
% cite works showing that clipping helps in non-smooth regions.
% PPO is kinda like clipping
% one requirement for SGDA/GDA is to have the policy side K-smooth and k-lipschitz


==> sections/citations.tex <==
\paragraph{Citations}
\begin{itemize}
    \item Zero-shot coordination. Attempt to improve upon self-play by adding other policies to the mix and breaking symmetries \citep{hu_other_play_zero_2020}. \citep{muglich_equivariant_networks_zero_2022} better ways to break symmetries pluggable to NNs.
    \item Zero-shot generalisation / Ad-hoc teamwork / Zero-shot transfer to new co-player. Hanabi with humans \citep{hu_other_play_zero_2020}. \citep{leibo_scalable_evaluation_multi_2021, agapiou_melting_pot_2_2023} show that cross-play (XP) with VMPO/A3C with joint rewards is usually not enough to learn robust policies, serves as "default" empirical evaluation for zero-shot generalisation. \citep{barrett_empirical_evaluation_ad_2011} first empirical evaluation of zero-shot generalisation. 
    \item Beginnings of Ad hoc Teamwork, \citep{bowling_coordination_adapatation_impromptu_2005, rovatsos_towards_social_complexity_2002}. 2022 survey on ad-hoc teamwork, \citep{mirsky_survey_ad_hoc_2022} ("All agents are assumed to have a common objective, but some teammates might have additional, individual objectives, or even completely different rewards").
    \citep{albrecht_empirical_study_practical_2015} proposes way to adapt to policy types using pseudo-bayesian beliefs..
     \citep{muglich_generalized_beliefs_cooperative_2022} similar (must look deeper into the differences). \citep{stone_ad_hoc_autonomous_2010} formalizes the problem as a challenge, and pushes the community to work on ad-hoc teamwork generalisation, gives good examples.
    \item Zero-shot domain adaptation. \citep{higgins_darla_improving_zero_2017}. \citep{schafer_task_generalisation_multi_2022} task generalisation in MARL. \citep{garcin_how_level_sampling_2023} observes the necessity to have a precise distribution over "scenarios", here they describe it as tasks, they also compare with unsupervised environment design. 
    \item How to evaluate/quantify generalization in RL.\citep{cobbe_quantifying_generalization_reinforcement_2019}. Scenario at test time should be different from train time. -> achievable with other policies.
    \item Human-AI cooperation. 
    \item Minimax-Bayes \citep{berger_statistical_decision_theory_1985}
    \item Diverse policy generation for ad-hoc teamwork. \citep{canaan_generating_adapting_diverse_2023} uses rule based policies generated with MAP-elites. \citep{muglich_generalized_beliefs_cooperative_2022} uses GA with simple NN policies. \citep{lupu_trajectory_diversity_zero_2021} through regularisation. \citep{jaderberg_human_level_performance_2019} reward shaping
    \item plastic algorithms ? \citep{barrett_cooperating_unknown_teammates_2015, barrett_making_friends_fly_2017}
    \item model based RL for both env and policies (ad hoc generalisation) \citep{ribeiro_teamster_model_based_2023}
    \item overfitting to policies encountered during training. \citep{lanctot_unified_game_theoretic_2017}
    \item Collaborating with Humans without Human Data -> training policies independently to break symmetries
    \item best response to populations \citep{lupu_trajectory_diversity_zero_2021, strouse_collaboration_with_humans_2021}
    \item the challenge of the ZSC framework arises from the fact that
many collaborative settings admit multiple joint-strategies
that are optimal under self-play (SP) (Tesauro, 1994) yet
incompatible. Thus, if we naively train two independent
agents in SP, there is no guarantee that they will converge to
compatible policies.
\end{itemize}

==> sections/future.tex <==
\paragraph{Future Directions}
Future direction -> "auto" curriculum learning (over partners, not env) for AHT/MARL.

==> sections/limitations.tex <==
\paragraph{Limitations}
[When using utility, if for some scenario, the maximum utility was reached, but its utility is still lower the other scenarios, then we are stuck learning forever on the same scenario, while there is possibly some possible improvements on other scenarios without degrading the performance on this scenario.]

[With utility, the adaptive distribution may set the probability of hardest scenarios (scenarios where it is difficult to learn) to the highest in early stages of learning, which is quite the contrary to what you typicially do in curriculum learning.]

[Only experiment with two players]
[Need tests on other domains]



==> sections/notes.tex <==
% propose BF GDA/SGDA
% introduce adaptive regret notion and non-degenerative populations
%%% theoretical results
% convergence of GDA/SGDA in our setting for exponential policies
% hypotethis that it should work still by clipping the policy side ( then experiments), then argue that it can help for convergence of NN policies (talk about L0-L1 smoothness and past results on that matter, theoretical results left for future work on GDA/SGDA)
% 
%%% experiments
% repeated prisonner's dilemma as a first example to show results on GDA, (with specific or full set of deterministic policies??)
% Show clipping effect (works on higher lr)
% boxplots, learned distributions, learning curve on worst-case regret ?

% more advanced experiments on random POMDPS (provide figure for the env ?)
% show empirically that it still works. clipping as well ?

% final set of experiments on complex environments with NN policies.
% > leduc poker, melting pot
% > cooperation on mujoco tasks (say the "human" controls a part of the robot, and the agent assists)

==> sections/old_proofs.tex <==
\begin{proof}[Proof of Lemma~\ref{lemma:scenario_equivalence_regret}]
    Let $\scenario$ be a scenario in $S$. $\scenarioset$ is an $\epsilon$ net for $S$, then there must exist a scenario $\scenario'$ such that $d(\scenario, \scenario')<\epsilon$.
    Naturally, we have $\forall s\in\states, i\in[1,\dots, c]$,
    \begin{align}
        |\max_{\afocal} [\rewardfunc_\scenario(s, \afocal, i)]- \max_{\afocal} [\rewardfunc_{\scenario'}(s, {\afocal}, i)]| &\leq 
        \max_{\afocal} |\rewardfunc_\scenario(s, \afocal, i)-\rewardfunc_{\scenario'}(s, {\afocal}, i)|\\
        & < \epsilon\rmax,
    \end{align}
    where the last inequality was proven in the above proof, in equation \eqref{eq:reward_similarity}.
    Again, using the same results and notations from the above proof, having $U^*_t(\scenario, s)$ denote the optimal utility of scenario $\scenario$ at timestep $t$ and state $s$, we prove by induction that:
    \begin{equation}
        \forall t \in [1\dots T], \forall s \in \states, |U^*_t(\scenario, s)-U^*_t(\scenario', s)| < \epsilon\rmax (T-t+1)(T-t)/2.
    \end{equation}
    At $t = T$, we have:
        \begin{align}
         & |U^*_T(\sigma, s) - U^*_T(\sigma', s)| \\
         &= |\max_{\afocal} [\dfrac{1}{c}\sum_i^c\big[\rewardfunc_\scenario(s, \afocal, i)] - \max_{\afocal}[\rewardfunc_{\scenario'}(s, \afocal, i)]| \\
         & < \epsilon\rmax.
        \end{align}

    At last, noticing that $|R(\pi, \scenario) - R(\pi, \scenario')| \leq |U^*(\scenario) - U^*(\scenario')| + |U(\pi, \scenario) - U(\pi, \scenario')| < \epsilon T^2\rmax$ concludes the proof.
    
\end{proof}
